Towards CO2 valorization in a multi remote renewable energy hub framework

In this paper, we propose a multi-RREH (Remote Renewable Energy Hub) based optimization framework. This framework allows a valorization of CO2 using carbon capture technologies. This valorization is grounded on the idea that CO2 gathered from the atmosphere or post combustion can be combined with hydrogen to produce synthetic methane. The hydrogen is obtained from water electrolysis using renewable energy (RE). Such renewable energy is generated in RREHs, which are locations where RE is cheap and abundant (e.g., solar PV in the Sahara Desert, or wind in Greenland). We instantiate our framework on a case study focusing on Belgium and 2 RREHs, and we conduct a techno-economic analysis. This analysis highlights the key role played by the cost of the two main carbon capture technologies: Post Combustion Carbon Capture (PCCC) and Direct Air Capture (DAC). In addition, we use our framework to derive a carbon price threshold above which carbon capture technologies may start playing a pivotal role in the decarbonation process of our industries. For example, this price threshold may give relevant information for calibrating the EU Emission Trading System so as to trigger the emergence of the multi-RREH.

==> text/Modelling.tex <==
\section{Modelling}
\label{fig:Modelling}

This section describes the core of our methodology, a linear program (LP). The LP is modelled using a recently proposed framework, the Graph-Based Optimization Modeling Language (GBOML) that we present in section \ref{subsec:GBOML}. The LP formalization is provided in section \ref{subsec:modellingAssumptions}.

\subsection{GBOML}
\label{subsec:GBOML}

    In this work, we rely on a the Graph-Based Optimization Modelling Language (GBOML), a recently developed framework for enhancing the modelling of energy systems \cite{Miftari2022}. One key aspect when using GBOML is to divide the model into nodes and clusters; in our case, we consider the following nodes: on-shore Belgium, off-shore Belgium, and as many RRH as desired.
    
    The Belgian on-shore node models energy demands, CO2 emissions, PCCC and export of CO2. The RREH handles imports of CO2, production of H$_2$ from renewable energy, transformation of CO2 into CO2 neutral synthetic CH$_4$.


\subsection{Main modelling Assumptions}
\label{subsec:modellingAssumptions}


\subsubsection{Objective}
\label{subsub:objective}

    The objective function of the model is obtained by summing costs associated with all technologies and carriers involved in the model.
    
    Minimize the overall costs function (Capex, Opex, Energy not served, $CO_2$ emissions).

\subsection{CO2 emitters}
    \label{sub:CO2_emitters}
    
    The energy demand center includes several $CO_2$ emitters, mainly gas fired power plants and industries. Such quantities of $CO2_2$ are captured using PCCC technologies. 
    
    We denote by $\mathcal{P}_{CO_2}$ the set of all technologies that emit CO2 and that may be equiped with PCCC technologies.
    
    Each CO2 emitter is modelled according to the following characteristics:
    \begin{itemize}
        \item CO2 emission curve, in CO2 kt/h, $q^{CO_2,(i)}_t$, where $i \in \{ 1, \ldots , N^{CO_2}  \}$ indexes CO2 emitters, \textcolor{red}{Victor note: in \cite{BERGER_power_to_gas_2020106039} the notation is $Q^{p}_{CO_2, t}$ with $p \in \mathcal{P}_{CO_2}$ is there a reason to not follow the notation of Mathias? }
        \item For each CO2 emitter , there is the possibility to capture CO2 using PCCC technologies.
    \end{itemize}



\subsection{CO2 capture}

    Two main carbon capture processes are considered in this paper: Post Combustion Carbon Capture (PCCC) and Direct Air Capture (DAC).
    
    Different PCCC technologies exist, but absorption solvent-based methods is currently the leading one \cite{madejski2022methods}. It is based on a reaction between CO2 and a solvent in aqueous solution. The capture is achieved in a two-step process. In the first step, the post-combustion gas reacts with the solvent in order to catch the carbon dioxyde. In the second step, the $CO_2$ is regenerated at high temperature in a stripper.
    
    PCCC is modelled using the following characteristics:
    \begin{itemize}
        \item $\Phi^{p,CC}$: Electrical energy required per unit mass of CO2 captured via PCCC for technology $p \in \mathcal{P}_{CO_2}$.
        \item $Q^{c, CC}_{CO_2,t}$: fraction of CO2 mass flow of technology $p \in \mathcal{P}_{CO_2}$ captured via PCCC at time $t \in \{ 0, \ldots, T-1  \}$.
    \end{itemize}
    
    
    Direct Air Capture technologies are mainly divided into two categories: (i) high temperature aqueous solutions and (ii) low temperature solid sorbent systems \cite{fasihi2019techno}, the latter showing lower heat supply costs.
    
    DAC is modelled using the following characteristics:
    
    \begin{itemize}
        \item $\Phi^{DAC}_E$: Electrical energy required per unit mass of CO2 captured using DAC [GWh/kt]. 
        \item $\Phi^{DAC}_{NG}$: Natural gas energy required per unit mass of CO2 captured using DAC [GWh/kt].
        \item $Q^{DAC}_{CO_2, t}$: CO2 mass flow exiting DAC units at time $t \in \{ 0, \ldots, T-1  \}$ [kt/h].
        \item $Q^{DAC, A}_{CO_2, t}$: CO2 mass flow captured from the atmosphere via DAC at time $t \in \{ 0, \ldots, T-1  \}$ [kt/h].
    \end{itemize}
    


\subsubsection{Remote Renewable Energy Hubs}
\label{subsub:RREH}

    We denote by $\mathcal H$ the set of all RREH. Each hub $h \in \mathcal{H}$ is characterised using the following characteristics:
    \begin{itemize}
        \item Renewable energy resources, modelled in the form of capacity factor time series $\pi^{PV,h}_t$ (for solar PV) and $\pi^{W,h}_t$ (for wind energy) 
        \item Electrolysis and methanation plants. \textcolor{red}{Victor Note: cfr equations 17 to 21 and eq 28 to 31 in \cite{BERGER_power_to_gas_2020106039}}
        \item Geographical characteristics, including distance to the Energy Demand Center  $d^{h} \in \mathbb{R}$.
    \end{itemize}
    
    
    
    
    Many constraints associated with renewable energy generation, 


\subsubsection{CO2 and Synthetic methane transportation}
    Carriers : Pipes and boats.
    
    
    In this first version of our model, we assume a simplified version of the CO2 transportation system by considering a continuous flow between the RREHs and the energy demand center.

\subsubsection{Decision variables}
\label{subsub:carriers}

    Among variables to be optimised, there are both sizing and operation variables. Sizing variables relates with investment decision variables.
    
    how large generation and transport capacities should be sized. 

\subsubsection{Main cost assumptions}

    PCCC and DAC costs, as well as CO2  transportation costs, play a key role in our results.

==> text/annex.tex <==
\subsection{Previous scenari}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
            \hline
            scenario & time horizon & Cap on CO2 & Cost of CO2 & ENS ALLOWED & Cost ENS & Pipe and/or Boat & Objective \\ \hline
            1 & 8760 & 0.0 & 0.0 & False & - & pipe and boat & 39992.71 \\
            2 & 8760 & None & 0.08 & True & 3.0 & pipe and boat & 37515.28 \\
            3 & 8760 & None & 0.0 & True & 3.0 & pipe and boat & 36107.64 \\
            4 & 8760 & None & 0.08 & True & 3.0 & only pipe & 37552.58 \\
            5 & 8760 & None & 0.08 & True & 3.0 & only carrier & 37539.88 \\
            6 & 8760 & 0.0 & 0.0 & False & - & pipe and boat & 52345.09 \\
            7 & 8760 & None & 0.08 & False & - & pipe and boat & 39050.49 \\
            8 & 8760 & None & 0.1648981 & False & - & pipe and boat & 39992.71 \\
            \hline
            
    \end{tabular}
    \caption{Scenari parameters}
    \label{tab:scenario_parameters_prev}
\end{table}


\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
         \hline
            scenario & wind on & wind off & solar\_be & ccgt\_be & wind\_gl & wind\_nz & solar\_nz \\ \hline
            1 & 8.40 & 7.71 & 9.56 & 22.41 & 0.00 & 98.13 & 91.39 \\ 
            2 & 8.40 & 8.00 & 13.83 & 17.39 & 0.00 & 87.31 & 81.09 \\ 
            3 & 8.40 & 8.00 & 13.29 & 17.32 & 0.00 & 86.46 & 80.49 \\ 
            4 & 8.40 & 8.00 & 13.42 & 17.30 & 0.00 & 86.42 & 80.45 \\ 
            5 & 8.40 & 8.00 & 13.88 & 17.50 & 0.00 & 87.93 & 81.63 \\ 
            6 & 8.40 & 8.00 & 15.68 & 19.58 & 126.54 & 0.00 & 0.00 \\ 
            7 & 8.40 & 7.19 & 8.95 & 22.06 & 0.00 & 93.04 & 86.40 \\ 
            8 & 8.40 & 7.71 & 9.56 & 22.41 & 0.00 & 98.18 & 91.43 \\  
            \hline
            
    \end{tabular}
    \caption{Total Power installation in GW}
    \label{tab:power_prev}
\end{table}



\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
            \hline
            scenario & PCCC & PCCC CCGT & DAC NZ & DAC GR \\ \hline
            1 & 4.11 & 2.59 & 1.26 & 0.00 \\ 
            2 & 4.11 & 1.55 & 0.00 & 0.00 \\ 
            3 & 5.00 & 0.44 & 0.00 & 0.00 \\ 
            4 & 4.11 & 1.33 & 0.00 & 0.00 \\ 
            5 & 4.11 & 1.59 & 0.00 & 0.00 \\ 
            6 & 4.11 & 2.59 & - & 1.22 \\ 
            7 & 4.11 & 1.76 & 0.00 & 0.00 \\ 
            8 & 4.11 & 2.59 & 1.27 & 0.00 \\
            \hline
            
    \end{tabular}
    \caption{Technology of capture with capacity in kt/h}
    \label{tab:capture_co2_prev}
\end{table}


\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
            \hline
            Scenario & pipe nz & carrier nz & pipe gr & carrier gr \\
            \hline
            1 & 3.196 & 2.363 & 0.000 & 0.000 \\
            2 & 2.158 & 5.626 & 0.000 & 0.000 \\
            3 & 5.445 & 0.000 & 0.000 & 0.000 \\
            4 & 5.442 &  - & 0.000 &  - \\
            5 &  - & 9.280 &  - & 0.000 \\
            6 & 0.000 & 0.000 & 0.000 & 7.518 \\
            7 & 2.374 & 5.833 & 0.000 & 0.000 \\
            8 & 3.196 & 2.344 & 0.000 & 0.000 \\
            \hline
    \end{tabular}
    \caption{Transport technology with capacity in kt/h}
    \label{tab:transport_co2_prev}
\end{table}

\subsection{Technologies}\label{subsec:technologies}
In this sub-section, the different types of technologies are described, namely conversion and storage technology and balances (respectively represented by nodes and hyperedges in \autoref{sec:modelling}). The different constraints are also thouroughly described. The notation follows the convention taken in \cite{Berger2021} where the Latin letters denote optimisation variables and indices, while Greek letters indicate parameters. 

\subsubsection{Nodes}

% \textbf{Variable Energy Sources}: A set $\mathcal{P}_R = \{PV, W_{on}, W_{off}\}$:
    % $$
    % \begin{aligned}
    % & P_{E, t}^p \leq \pi_t^p\left(\kappa_0^p+K_E^p\right), \quad \forall t \in \mathcal{T}, \quad \forall p \in \mathcal{P}_R \\
    % & K_E^p \leq \kappa_{\max }^p, \quad \forall p \in \mathcal{P}_R
    % \end{aligned}
    % $$
    % with $\kappa_0^p$ represents the pre-installed capacity and $K_E^p$ the newly installed capacity. The parameter $\pi_t^p$ represents the load factor at timestep $t$. 
    % Investment and operating costs are described as
    % $$
    % C^p=\left(\zeta^p+\theta_f^p\right) K_E^p+\sum_{t \in \mathcal{T}} \theta_v^p P_{E, t}^p \delta t, \quad \forall p \in \mathcal{P}_R
    % $$
    % with 

% \textbf{Dispatchable Technologies}
    % \begin{equation}
        % \begin{aligned}
        % & P_{E, t}^p \leq \kappa_0^p+K_E^p, \quad \forall p \in \mathcal{P}_D \\
        % & P_{E, t}^p-P_{E, t-1}^p \leq \Delta_{+}^p\left(\kappa_0^p+K_E^p\right), \quad \forall p \in \mathcal{P}_D \\
        % & P_{E, t}^p-P_{E, t-1}^p \geq-\Delta_{-}^p\left(\kappa_0^p+K_E^p\right), \quad \forall p \in \mathcal{P}_D \\
        % & \mu^p\left(\kappa_0^p+K_E^p\right) \leq P_{E, t}^p, \quad \forall p \in \mathcal{P}_D \\
        % & Q_{\mathrm{CO}_2, t}^p=\frac{\nu^p P_{E, t}^p}{\eta^p}, \quad p \in\{\mathrm{BM}, % \mathrm{WS}\}
        % \end{aligned}
    % \end{equation}

\textbf{Conversion technologies}: 
Let us consider a given node $n \in \mathcal{N}$ wich is a conversion technology \textit{i.e.} which takes as input a given commodity $i$ flow and outputs another commodity $r$ flow. A conversion technology is described by an internal variable representing the capacity of a guven technology associated with a given commodity and by external variables linking the flows in and out. These relations are expressed as 

\begin{equation}
q_{rt}^n - \phi_{i}^n q_{i(t+\tau_{i}^n)}^n = 0, \mbox{ } \forall i \in \mathcal{I}^n\setminus\{r\}, \mbox{ } \forall t \in \mathcal{T}^n,
\label{eq:conversion}
\end{equation}
where $q_{it}^n \in \mathbb{R}^{+}$ is the flow of a given commodity $i$, $\phi_{i}^n$ is the conversion factor from $i$ to $r$ and $\tau_{i}^n$ is the time for the process to occur. Other constraints occur in conversion technology such as the maximum capacity expressed as

\begin{equation}
K_0^n - K_t^n = 0, \mbox{ } \forall t \in \mathcal{T}\setminus\{0\},
\label{eq:conversioncapacitystatic}
\end{equation}
where $K_t^n$ is the capacity at each time step of the time horizon considered. The maximum capacity remains constant over the entire horizon because we use a static investment policy. In the following $K^{n}$ will be a shorthand for $K_0^n$ and represents the new capacity installed. 

Some conversion technology are not dispatchable (\textit{e.g.} variable renewable energy). Therefore, the availability of such a technology is expressed as 

\begin{equation}
q_{r't}^n - \pi_{t}^n (\underbar{$\kappa$}^{n} + K^{n}) \le 0, \mbox{ } \forall t \in \mathcal{T},
\label{eq:sizing}
\end{equation}
where $\pi_{t}^n \in [0,1]$ is the normalized capacity factor of the technology $n$ at timestep $t$, $\underbar{$\kappa$}^{n}$ is the pre-installed capacity. 

Some technology capacities are bounded by a maximum potential capacity. This constraint reads as
\begin{equation}
(\underbar{$\kappa$}^{n} + K^{n}) - \bar{\kappa}^{n} \le 0,
\label{eq:potential}
\end{equation}
where $\bar{\kappa}^{n}$ is the maximum capacity of technology $n$.

To run a technology $n$ a minimal input flow may be needed and is expressed as
\begin{equation}
\mu^{n} (\underbar{$\kappa$}^{n} + K^{n}) - \frac{\phi_{i}^n}{\phi_{r'}^n}q_{it}^n \le 0, \mbox{ } \forall t \in \mathcal{T},
\label{eq:mustrun}
\end{equation}
where $\mu^{n} \in [0,1]$ represents the minimum operating level (as a fraction of the installed capacity). \textcolor{red}{Since the technology is sized with respect to the flow of commodity r', the flow of a commodity $i \neq r'$ must be scaled by the ratio of conversion factors in \ref{eq:mustrun}. }

Some conversion technologies are limited in the rate at which they can change a commodity flow. These are the so-called ramping up constraint defined as
\begin{equation}
\frac{\phi_{i}^n}{\phi_{r'}^n}(q_{it}^n - q_{i(t-1)}^n) - \Delta_{i,+}^{n} (\underbar{$\kappa$}^{n} + K^{n}) \le 0, \mbox{ } \forall t \in \mathcal{T}\setminus\{0\},
\label{eq:rampup}
\end{equation}

and ramping down constraint defined as
\begin{equation}
\frac{\phi_{i}^n}{\phi_{r'}^n}(q_{i(t-1)}^n - q_{it}^n) - \Delta_{i,-}^{n} (\underbar{$\kappa$}^{n} + K^{n}) \le 0, \mbox{ } \forall t \in \mathcal{T}\setminus\{0\},
\label{eq:rampdown}
\end{equation}
where $\Delta_{i,+}^{n} \in [0,1]$ and $\Delta_{i,-}^{n} \in [0,1]$ the maximum rates at which flows can be ramped up and down.

Finally, we get the local objective function for technology $n$ written as
\begin{equation}
F_n = \nu (\zeta^{n} + \theta_f^n) K^{n} + \sum_{t \in \mathcal{T}} \theta_{t,v}^n q_{r't}^n \delta t,\label{eq:objectiveconversion}
\end{equation}
where $\nu \in \mathbb{N}$ is the number of years spanned by the optimisation horizon, $\zeta^n \in \mathbb{R}_+$ represents the (annualised) investment cost (also known as capital expenditure, CAPEX), $\theta_f^n \in \mathbb{R}_+$ models fixed operation and maintenance (FOM) costs and $\theta_{t,v}^n \in \mathbb{R}_+$ represents variable operation and maintenance (VOM) costs, which may be time-dependent.


%%%%%%%%%%%%%%%
%   STORAGE   %
%%%%%%%%%%%%%%%

\textbf{Storage}: Let $n \in \mathcal{N}$ be a node representing a given storage technology. This later internal variable represents the current amount of commodity stored while the external variables are the flows in (charge) and out (discharge) of this technology as well as other commodity input flow needed. The dynamics of charge and discharge is described as follows

\begin{equation}
e_{t+1}^n - (1-\eta_{S}^n) e_{t}^n - \eta_{+}^{n} q_{it}^n + \frac{1}{\eta_{-}^{n}} q_{jt}^n = 0, \mbox{ } \forall t \in \mathcal{T} \setminus\{T-1\},
\label{eq:storagedynamics}
\end{equation}
where $e_{t}^n \in \mathbb{R}_+$ is the inventory level at time $t$, $q_{i_ut}^n \in \mathbb{R}_+$ and $q_{i_yt}^n \in \mathbb{R}_+$ represent commodity in and outflows at time $t$, respectively, $\eta_S^n \in [0, 1]$ is the self-discharge rate, $\eta_+^n \in [0, 1]$ is the charge efficiency and $\eta_-^n \in [0, 1]$ is the discharge efficiency. The consumption of other commodity may be modelled with

\begin{equation}
q_{lt}^n - \phi_{i}^n q_{it}^n = 0, \mbox{ } \forall t \in \mathcal{T}.
\label{eq:conversionstorage}
\end{equation}

To avoid board effect, we impose that the stock at the begininng of the time horizon is equal at the end of the time horzion. Thsi prevents the model to use freely a commodity stored. The constraint can be written as
\begin{equation}
e_{0}^n - e_{T-1}^n = 0.
\label{eq:storagecyclicity}
\end{equation}
where $e_{0}^n$ is the inventory level at timestep zero and $e_{T-1}^n$ is the inventory level at the end of the spanned time horizon. 

As for conversion technology (\textit{cfr} \autoref{eq:conversioncapacitystatic}) the policy of investment is static. Thus it can be expressed as 
\begin{equation}
E_0^n - E_t^n = 0, \mbox{ } \forall t \in \mathcal{T}\setminus\{0\},
\label{eq:storagestockstatic}
\end{equation}
where $E_0^n$ is the newly installed capacity. In the later, the shorthand $E^n$ to denote $E_t^n$ will be used. 
The total storage capacity is defined as

\begin{equation}
e_{t}^n - (\underbar{$\epsilon$}^{n} + E^{n}) \le 0, \mbox{ } \forall t \in \mathcal{T},
\label{eq:storagestocksizing}
\end{equation}

As stated in \autoref{eq:potential} for conversion technologies, storage technology might have a maximum storage capacity. This is expressed as 
\begin{equation}
(\underbar{$\epsilon$}^{n} + E^{n}) - \bar{\epsilon}^{n} \le 0,
\label{eq:storagepotential}
\end{equation}
where $\bar{\epsilon}^n \in \mathbb{R}_+$ represents the maximum stock capacity that may be deployed. 

A minimum inventory level may be used and described as follows


\begin{equation}
\sigma^{n}(\underbar{$\epsilon$}^{n} + E^{n}) - e_{t}^n \le 0, \mbox{ } t \in \mathcal{T},
\label{eq:storageminimumsoc}
\end{equation}
where $\sigma^{n} \in [0, 1]$ is the mimum level of the inventory as a proportion of the installed capacity. 

The maximum inflow is modelled using an internal variable that is also constant throughout the time horizon considered, as in Eq. \eqref{eq:conversioncapacitystatic}. It is defined as follows
\begin{equation}
q_{it}^n - (\underbar{$\kappa$}^{n} + K^{n}) \le 0, \mbox{ } \forall t \in \mathcal{T},
\label{eq:storageflowplussizing}
\end{equation}
where $\underbar{$\kappa$}^n \in \mathbb{R}_+$ denotes the existing flow capacity and $K^n \in \mathbb{R}_+$ is used as shorthand for the new capacity. The maximum in- and outflows may be asymmetric, depending on the properties of the underlying technology, which is modelled via
\textcolor{red}{The maximum in- and outflows may be asymmetric, depending on the properties of the underlying technology, which is modelled via}
\begin{equation}
q_{jt}^n - \rho^{n} (\underbar{$\kappa$}^{n} + K^{n}) \le 0, \mbox{ } \forall t \in \mathcal{T},
\label{eq:storageflowminussizing}
\end{equation}
where $\rho^n \in \mathbb{R}_+$ represents the maximum discharge-to-charge ratio.
Finally the local objective for node $n$ can be written as follows
\begin{equation}
F^n = \Big[\nu (\varsigma^{n} + \vartheta^{n}_{f}) E^{n} + \sum_{t \in \mathcal{T}} \vartheta_{t,v}^n e_{t}^n\Big] + \Big[\nu (\zeta^{n} + \theta^n_f) K^{n} + \sum_{t \in \mathcal{T}} \theta_{t,v}^n q_{it}^n \delta t \Big].
\label{eq:objectivestorage}
\end{equation}
where $\varsigma^n \in \mathbb{R}_+$ and $\zeta^n \in \mathbb{R}_+$ represent the stock and flow components of CAPEX, $\vartheta_f^n \in \mathbb{R}_+$ and $\theta_f^n \in \mathbb{R}_+$ model the stock and flow components of FOM costs, while $\vartheta_{t,v}^n \in \mathbb{R}_+$ and $\theta_{t,v}^n \in \mathbb{R}_+$ represent the stock and flow components of VOM costs, which may be time-dependent.

\subsubsection{Hyperedges}
\textbf{Conservation}: Let $e\in \mathcal{E}$ be a conservation hyperedge which ensure that all the flows going in and out of a given commodity are respected. 
\begin{equation}
\sum_{n \in e_T} q_{it}^n - \sum_{n \in e_H} q_{it}^n - \lambda_{t}^e = 0, \mbox{ } \forall t \in \mathcal{T},
\label{eq:conservationhyperedge}
\end{equation}


